NARF22: Neural Articulated Radiance Fields for Configuration-Aware Rendering

Articulated objects pose a unique challenge for robotic perception and manipulation. Their increased number of degrees-of-freedom makes tasks such as localization computationally difficult, while also making the process of real-world dataset collection unscalable. With the aim of addressing these scalability issues, we propose Neural Articulated Radiance Fields (NARF22), a pipeline which uses a fully-differentiable, configuration-parameterized Neural Radiance Field (NeRF) as a means of providing high quality renderings of articulated objects. NARF22 requires no explicit knowledge of the object structure at inference time. We propose a two-stage parts-based training mechanism which allows the object rendering models to generalize well across the configuration space even if the underlying training data has as few as one configuration represented. We demonstrate the efficacy of NARF22 by training configurable renderers on a real-world articulated tool dataset collected via a Fetch mobile manipulation robot. We show the applicability of the model to gradient-based inference methods through a configuration estimation and 6 degree-of-freedom pose refinement task. The project webpage is available at: https://progress.eecs.umich.edu/projects/narf/.

==> sections/problem.tex <==
% PROBLEM STATEMENT

\ocj{use the level description provided in @stanlew presentation for group}
\ocj{include visual picture of what a NeRF does, similar to what stanlew showed in his presentation}
% The model for semi-synthetic dataset generation essentially needs to solve the novel-view synthesis problem, but modified to also include a configuration paramaterization component.

% More formally, the problem can be stated as: 
Given $N$ images ${\{P_{\text{rgb}^{(i)}}\}}$ containing a particular articulated object, the 6 degree-of-freedom (DoF) object poses in the camera frame ${\{X^{(i)}\}}$, the object configurations ${\{Z_i\}}$, and the image segmentations ${\{P_{\text{mask}^{(i)}}\}}$, we wish to determine a function $F$ that takes in a new 6-DOF pose and configuration ${(X_{\text{inf}}, Z_{\text{inf}})}$ and produces an estimated image output $P_{\text{inf}}$. $F$ is found by decreasing a loss function $L$ which compares the result of rendering an epipolar ray batch via $F$ to the corresponding pixels of the training image.
\henxu{Perhaps a few figures about P,X and Z could help to better understand the stated problem.}
\jana{discuss the ray thing}


%Put more succinctly, the image-synthesis task can be said to be as follows: \jana{I don't think this is the clearest way to put this. I'd just write out the loss and describe the image generation part separately}

%\begin{equation} \label{prob_statement}
%\begin{aligned}
%& \underset{i = 1, \ldots, N}{\text{minimize}}
%& & L(P_{rgb,i} * P_{mask,i} , P_{inference,i}) \\
%& \text{subject to}
%& & P_{inference,i} = F(P_{rgb,i} * P_{mask,i}, Z_i, X_i)\\\\
%& & & i=1,\ldots,N \text{ is not in the training set}
%\end{aligned}
%\end{equation}

